The Size Evolution of Elliptical Galaxies

Recent work has suggested that the amplitude of the size mass relation of massive early type galaxies evolves with redshift. Here we use a semi-analytical galaxy formation model to study the size evolution of massive early type galaxies. We find this model is able to reproduce the amplitude of present day amplitude and slope of the relation between size and stellar mass for these galaxies, as well as its evolution. The amplitude of this relation reflects the typical compactness of dark halos at the time when most of the stars are formed. This link between size and star formation epoch is propagated in galaxy mergers. Mergers of high or moderate mass ratio (less than 1:3) become increasingly important with increasing present day stellar mass for galaxies more massive than $10^{11.4}M_{\odot}$. At lower masses, low mass ratio mergers play a more important role. In situ star formation contribute more to the size growth than it does to stellar mass growth. We also find that, for ETGs identified at $z=2$, minor mergers dominate subsequent growth both for stellar mass and in size, consistent with earlier theoretical results.

==> macros_xie.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%macros for tex
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\dd}{{\rm d}}
\newcommand{\solarmass}{ \rm M_\odot}
\newcommand{\kpch}{h^{-1} \rm Kpc~}
\newcommand{\pch}{h^{-1} \rm pc~}
\newcommand{\mpch}{h^{-1} \rm Mpc~}
\newcommand{\msub}{m_{\rm sub}~}
\newcommand{\macc}{m_{\rm acc}~}
\newcommand{\mmsub}{m_{\rm sub}/M_{h}~}
\newcommand{\mmacc}{m_{\rm acc}/M_{h}~}
\newcommand{\muone}{\widetilde{\mu_1}}
\newcommand{\Mh}{M_{\rm h}}
\newcommand{\Rh}{R_{\rm h}}
\newcommand{\Vh}{V_{\rm h}}
\newcommand{\zh}{z_{\rm h}}
\newcommand{\omegam}{\Omega_{\rm m}}
\newcommand{\omegal}{\Omega_{\rm \Lambda}}
\newcommand{\omegab}{\Omega_{\rm b}}
\newcommand{\rvir}{r_{\rm vir}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\gsim { \lower .75ex \hbox{$\sim$} \llap{\raise .27ex \hbox{$>$}}}
\def\lsim { \lower .75ex \hbox{$\sim$} \llap{\raise .27ex \hbox{$<$}}}


